Toward Human-Quantum Computer Interaction: Interface Techniques for Usable Quantum Computing

By leveraging quantum-mechanical properties like superposition, entanglement, and interference, quantum computing (QC) offers promising solutions for problems that classical computing has not been able to solve efficiently, such as drug discovery, cryptography, and physical simulation. Unfortunately, adopting QC remains difficult for potential users like QC beginners and application-specific domain experts, due to limited theoretical and practical knowledge, the lack of integrated interface-wise support, and poor documentation. For example, to use quantum computers, one has to convert conceptual logic into low-level codes, analyze quantum program results, and share programs and results. To support the wider adoption of QC, we, as designers and QC experts, propose interaction techniques for QC through design iterations. These techniques include writing quantum codes conceptually, comparing initial quantum programs with optimized programs, sharing quantum program results, and exploring quantum machines. We demonstrate the feasibility and utility of these techniques via use cases with high-fidelity prototypes.

==> figures/alt-text.tex <==
Figure 1: "There are three parts. A, quantum mechanical properties, superposition, entanglement, and interference. B, example quantum gates: Hadamard, Rotation, and C-Not gates and their output probabilities. C, an example quantum circuit for entanglement or bell state, with a Hadamard gate on qubit A, and a C-Not gate on qubits A and B, resulting in state 500 zero-zero state and 500 one-one state."

Table 1: "A summary table for the present work and quantum computing tools: qiskit, cirq, qu-tip, strawberry fields, penny lane, braket, cuda-q, zaure, q-braid, classi-q."

Figure 2: "Four visualization cases for quantum computing. A, Classi-q's interactive whiteboard for quantum circuits. B, Bloch spheres for a qubit's state. A block sphere has three axes: x, y, and z. C, qiskit's machine dashboard. D, measurement histogram."

Figure 3: "QC interaction technique overview in terms of tasks and design principles."

Figure 4: "Problem-specific outcome visualizations. (A) state vector bit strings are replaced with the corresponding natural numbers in a measurement histogram. (B) State vector bit strings are divided and shown in a truth table view. (C) Measurement outcomes are reformatted as an image, with configuration options. (D) Contingency table for categorical data exploration which can be pivoted by qubits."

Figure 5: "Hypothetical error adjustment visualization example, comparing outcomes for reliable, less reliable, and nearly random measurements."

Figure 6: "The first case study for learning Shor's algorithm, part 1. (A) Writing a Shor's algorithm circuit. A1. Loading the circuit writer interface on Jupyter Notebook. A2. Specifying a circuit via the writer interface. A3. Generated circuit code in Qiskit. (B) Passing the job to IBM Q Cloud. B1. Set a real QPU, chosen by IBM. B2. Updated run code for a real QPU."

Figure 7: "The first case study for learning Shor's algorithm, part 2. (C). Saving and retrieving the job results. C1. Python codes for importing and saving the job data as a JSON file. C2. Python codes for retrieving the saved JSON file. C3. Loading a result viewer on a Jupyter Notebook. (D) Retrieving historical QPU data with a visualization."

Figure 8: "The second case study for quantum machine learning. (A) Writing a image convolution circuit. (B). Checking the outcome image with interactive configuration options."

Figure 9: "The third case study for circuit optimization, part 1. (A) Manually writing a Toffoli circuit. (B) Machine explorer interface for machine selection. B1. Loading a machine information dashboard. B2. Select decoherence times of qubits (T1 and T2). B3. Select basis gates. B4. Generate a reusable code snippet to extract the same information from different machines. B5. Extract the same information from other candidate machines."

Figure 10: "The third case study for circuit optimization, part 2. (C) Comparing different optimization strategies. C1. Passing different optimization strategies. C3. Displaying the optimization outcomes in a single dashboard with a summary table and cross-highlighting interaction for the differences in them."

Figure 11: "The third case study for circuit optimization, part 3. (D) executing the circuit. Once, the circuit is run on the specified simulators, the job data objects are post-processed and hypothetically error-adjusted measurement outcomes are generated. (E) Hypothetical error adjustment visualization. E1. Vigo simulator. E2. Bogota simulator. Note The hypothetical error adjustment shows that the Bogota simulator exhibits more erroneous output although both does not impact the interpretation of the outcome too much."

